Clinical trial site matching with improved diversity using fair policy learning

The ongoing pandemic has highlighted the importance of reliable and efficient clinical trials in healthcare. Trial sites, where the trials are conducted, are chosen mainly based on feasibility in terms of medical expertise and access to a large group of patients. More recently, the issue of diversity and inclusion in clinical trials is gaining importance. Different patient groups may experience the effects of a medical drug/ treatment differently and hence need to be included in the clinical trials. These groups could be based on ethnicity, co-morbidities, age, or economic factors. Thus, designing a method for trial site selection that accounts for both feasibility and diversity is a crucial and urgent goal. In this paper, we formulate this problem as a ranking problem with fairness constraints. Using principles of fairness in machine learning, we learn a model that maps a clinical trial description to a ranked list of potential trial sites. Unlike existing fairness frameworks, the group membership of each trial site is non-binary: each trial site may have access to patients from multiple groups. We propose fairness criteria based on demographic parity to address such a multi-group membership scenario. We test our method on 480 real-world clinical trials and show that our model results in a list of potential trial sites that provides access to a diverse set of patients while also ensuing a high number of enrolled patients.

==> figures/dummy.tex <==
\textbf{Case study 1: Trial No. NCT04369053} \\
This is a clinical trial related to studying the prevention of Colorectal Cancer Through Multiomics Blood Testing (PREEMPT CRC).


In Figure \ref{fig:145_perf}, we illustrate the change in the group representations between the set of investigators that have the highest enrollment, as compared to the list of K investigators from our model. 

\begin{figure}
    % \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[scale=0.23]{figures/145/base.png}
         \caption{}
         \label{fig:145_base_rep}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[scale=0.23]{figures/145/model.png}
         \caption{}
         \label{fig:145_model_rep}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[scale=0.23]{figures/145/rel_change.png}
         \caption{}
         \label{fig:145_rel_change}
     \end{subfigure}
        \caption{Average model performance in improving group representation for trial NCT04369053 . }
        \label{fig:145_perf}
\end{figure}


\begin{figure}
    % \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[scale=0.23]{figures/246/base.png}
         \caption{}
         \label{fig:246_base_rep}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[scale=0.23]{figures/246/model.png}
         \caption{}
         \label{fig:246_model_rep}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[scale=0.23]{figures/246/rel_change.png}
         \caption{}
         \label{fig:246_rel_change}
     \end{subfigure}
        \caption{Average model performance in improving group representation for trial  NCT02104817. }
        \label{fig:246_perf}
\end{figure}

\begin{figure}
    % \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[scale=0.23]{figures/556/base.png}
         \caption{}
         \label{fig:556_base_rep}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[scale=0.23]{figures/556/model.png}
         \caption{}
         \label{fig:556_model_rep}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[scale=0.23]{figures/556/rel_change.png}
         \caption{}
         \label{fig:556_rel_change}
     \end{subfigure}
        \caption{Average model performance in improving group representation for trial  NCT03255096. }
        \label{fig:556_perf}
\end{figure}



Let us also explore \textbf{how} such a change is brought about in group representation. Let us consider the set of investigators that were \textbf{dropped} from the top-K list and the set of investigators that were \textbf{added} to the top-K list based on diversity constraints. We list the location of these investigators, along with the demographic information from that location in Table \ref{tab:rel_change_enroll1}. As can be seen, the model chooses investigators from locations with a more diverse demographics.

\begin{table*}[h]
\begin{center}
\caption{Changes in the selected list of investigator locations for trial NCT04369053}
\label{tab:rel_change_enroll1}
    % \resizebox{\textwidth}{!}{
    \begin{tabular}{l|cccccc}
        \toprule
        Investigators (locations) \textbf{dropped} & White & Hispanic & Black & Asian & Mixed & Others \\
        \midrule
        Shreveport, LA & 78.6& \textbf{3.7}& \textbf{11.4}& \textbf{3.5}& 2.4& 0.5 \\
        Springfield, IL &77.0& \textbf{1.7}& \textbf{16.8}& \textbf{1.1}& 2.8& 0.6\\
         \bottomrule
         \toprule
        Investigators (locations) \textbf{added} & &  &  & &  &  \\
        \midrule
        Portland, OR &61.2& \textbf{12.2}& \textbf{8.4}& \textbf{11.9}& 4.3& 2.0\\
        Union, NJ &42.3& \textbf{17.3}& \textbf{26.3}&\textbf{10.9}& 0.9& 2.4\\
        \bottomrule
    \end{tabular}
    % }
\end{center}
\end{table*}

\begin{figure}[h]
    \centering
    \includegraphics[scale = 0.6]{figures/145/map.png}
    \caption{Illustration of the top-K investigators chosen with and without the diversity constraints, for trial NCT04369053 . Notice that the model chooses to replace two of the investigators to achieve a more diverse patient cohort.}
    \label{fig:145_map}
\end{figure}



In Figure \ref{fig:145_map}, we illustrate the set of top-K investigators that have the highest patient enrollment for this trial, and the list of top-K investigators that were chosen by our model to account for the diversity constraints. Notice that the two lists have 8 investigators in common. This leads to a high expected enrollment from our model. Further, by replacing two of the investigators, our model achieves a significant increase in the diversity of the patient cohort.



\textbf{Case study 2: Trial No. NCT02104817} This is a clinical trial for testing a treatment for Atherosclerotic Cardiovascular Disease (CVD).




\begin{table*}[h]
\begin{center}
\caption{Changes in the selected list of investigator locations for trial  NCT02104817}
\label{tab:rel_change_enroll2}
    % \resizebox{\textwidth}{!}{
    \begin{tabular}{l|cccccc}
        \toprule
        Investigators (locations) \textbf{dropped} & White & Hispanic & Black & Asian & Mixed & Others \\
        \midrule
        Danville, PA &91.8& \textbf{2.6}& \textbf{1.8}& 3.3& 0.5& 0.0 \\
        Winston-Salem, NC &47.2& 14.3& 34& 2& 1.9& 0.6\\
        Fort Wayne, IN &91.9& \textbf{2.5}&\textbf{2.7}& 2.0& 0.8& 0.2\\
         \bottomrule
         \toprule
        Investigators (locations) \textbf{added} & &  &  & &  &  \\
        \midrule
        Wilmington, NC&47.1& 7.8& \textbf{41.3}& 0.4& 2.2&1.2\\
        Miami, FL&5.2& \textbf{91.9}&2.2& 0.4&0.2& 0.0\\
        Champaign, IL &67.1& 3.4& 9.6& 17.7& 1.9& 0.2\\
        \bottomrule
    \end{tabular}
    % }
\end{center}
\end{table*}

\begin{figure}[h]
    \centering
    \includegraphics[scale = 0.6]{figures/246/map.png}
    \caption{Illustration of the top-K investigators chosen with and without the diversity constraints, for trial NCT02104817.}
    \label{fig:145_map}
\end{figure}

In Figure \ref{fig:246_perf}, we illustrate the change in the group representations between the set of investigators that have the highest enrollment, as compared to the list of K investigators from our model. 
Let us also explore \textbf{how} such a change is brought about in group representation. Let us consider the set of investigators that were \textbf{dropped} from the top-K list and the set of investigators that were \textbf{added} to the top-K list based on diversity constraints. We list the location of these investigators, along with the demographic information from that location in Table \ref{tab:rel_change_enroll2}. As can be seen, the model chooses investigators from locations with a more diverse demographics.


\textbf{Case study 3: Trial No. NCT03255096 } This is a trial to study the impact of a drug to treat Diffuse Large B-cell Lymphoma and
High-Grade B-cell Lymphoma.


In Figure \ref{fig:556_perf}, we show the resulting group representations before and after imposing diversity constraints. Notice that there is not much change in the group representation among the top-K list of investigators. When we looked into the dataset for this trial, we found that the list of $M$ investigators provided to the algorithm did not provide a lot of room for improvement in the group composition. We provide more details below. 

In Table. \ref{tab:556_perf}, we list the $M=20$ investigators provided to the model in the order of \textbf{decreasing expected patient enrollment}. Without diversity constraints, the model would choose the top-10 locations, as \textbf{indicated in the Table in bold}. When diversity constraints are included, the model could potentially improve the group representation by choosing from locations with more than average representation for the underrepresented communities, highlighted with an asterisk (*) in the Table. Our model chooses to include Akron, OH and Oklahoma, OK in the top-10 list when diversity constraints are included. The locations towards the bottom of the Table would lead to a large decrease in expected patient enrollment and are hence not included in the selection.

\begin{table*}[h]
\begin{center}
\caption{List of 20 investigators presented to the model for ranking the top-10 for trial NCT03255096 }
\label{tab:556_perf}
    % \resizebox{\textwidth}{!}{
    \begin{tabular}{l|cccccc}
        \toprule
        Investigators (locations) & White & Hispanic & Black & Asian & Mixed & Others \\
        \midrule
\textbf{Charlotte, NC} &70.2&2.9&19.5& 3.8& 2.7& 0.9\\
\textbf{New York, NY}&78.4& 7.2& 1.3& 9.5& 2.7& 0.9\\
\textbf{Dallas, TX}&29.2& 41.1& 24.6& 3.3& 1.5&0.3\\
\textbf{Sandy, UT} &79.8& 13.5& 1.0& 3.2& 1.4& 1.1\\
\textbf{Canton, OH} &85.0& 2.0& 6.6& 0.4& 5.5& 0.5\\
\textbf{Columbus, GA} &63.8& 6.1& 22.6& 4.0& 2.6& 0.9\\
\textbf{Miami, FL} &14.0& 81.7& 2.1& 1.4& 0.7& 0.1\\
\textbf{Lexington, KY}&59.5& 4.7& 27.5& 4.2& 3.6& 0.4\\
\textbf{Worcester, MA} &57.4& 19.3& 13.6&7.1& 1.9&0.7\\
\textbf{Memphis, TN} &85.1& 2.7& 3.8& 6.5& 1.7& 0.3\\
{\color{blue}Akron, OH} \textbf{*}  &65.7& 4.8& 21.2& 0.7& 7.6& 0.0\\
{\color{blue}Oklahoma City, OK}\textbf{*} &60.4& 7.0& 23.8& 1.5& 5.6& 1.7\\
New York, NY &78.4& 7.2& 1.3& 9.5& 2.7& 0.9\\
Owensboro, KY &88.1& 2.9& 4.9& 2.1& 1.7& 0.3\\
Lincoln, NE &92.6& 0.9& 1.8& 3.1& 1.2& 0.4\\
Hollywood, FL \textbf{*}&52.2& 30.4& 13.3& 2.1& 1.6& 0.4\\
Panama City, FL &72.5& 7.4& 13.8& 1.8& 3.6& 0.9\\
Nashville, TN &73.2&6.7&15.2&2.5&1.9&0.5\\
Springfield, MO &90.6& 2.6& 2.4& 1.4& 2.1& 0.9\\
Pittsburgh, PA\textbf{*} &66.7& 2.2& 26.0& 1.5& 3.1& 0.6\\
\bottomrule
    \end{tabular}
    % }
\end{center}
\end{table*}

